Counterfactual Evaluation of Treatment Assignment Functions with Networked Observational Data

Counterfactual evaluation of novel treatment assignment functions (e.g., advertising algorithms and recommender systems) is one of the most crucial causal inference problems for practitioners. Traditionally, randomized controlled trials (A/B tests) are performed to evaluate treatment assignment functions. However, such trials can be time-consuming, expensive, and even unethical in some cases. Therefore, offline counterfactual evaluation of treatment assignment functions becomes a pressing issue because a massive amount of observational data is available in today's big data era. Counterfactual evaluation requires handling the hidden confounders -- the unmeasured features which causally influence both the treatment assignment and the outcome. To deal with the hidden confounders, most of the existing methods rely on the assumption of no hidden confounders. However, this assumption can be untenable in the context of massive observational data. When such data comes with network information, the later can be potentially useful to correct hidden confounding bias. As such, we first formulate a novel problem, counterfactual evaluation of treatment assignment functions with networked observational data. Then, we investigate the following research questions: How can we utilize network information in counterfactual evaluation? Can network information improve the estimates in counterfactual evaluation? Toward answering these questions, first, we propose a novel framework, \emph{Counterfactual Network Evaluator} (CONE), which (1) learns partial representations of latent confounders under the supervision of observed treatments and outcomes; and (2) combines them for counterfactual evaluation. Then through extensive experiments, we corroborate the effectiveness of CONE. The results imply that incorporating network information mitigates hidden confounding bias in counterfactual evaluation.

==> theo.tex <==
%and
%\begin{equation}
%	\pi_i^s(\bm{t}|\bm{x}_i;f)=\pi_i^s(\bm{t}'|\bm{x}_j;g) \; \text{if} \; r_i(f,\bm{t}) = r_i(g,\bm{t}')
%\end{equation}
%
\section{Theoretical Analysis of \textit{PLU}}
\label{sec:theo}
%
In this section, we begin by describing the conceptual objectives of the \textit{PLU} problem. Specifically, it leads to the optimal treatment outcomes by optimizing the objectives. Then we reveal their close connections to a subset of the functional space of ranking functions.


\vspace{-0.1in}
\subsection{Conceptual Objectives of \textit{PLU}}
In this subsection, we formally introduce the objective functions of the \textit{PLU} problem and carry out theoretical analysis to reveal the connection between the optimal solution of these objective functions and a subset of the space of ranking functions.
%

As discussed above, we have to consider the cases when the optimal treatment is not selected due to the preference of receivers. In this case, we still attempt to maximize the expected outcome in Eq.~\ref{eq:state}.
%
Thus, under the setting of deterministic preference, the objective function becomes:
\begin{equation}
\label{eq:obj2}
		\underset{f}{\arg\max}\; \frac{1}{N}\sum_{i=1}^N y_i(\hat{\bm{t}}_i^*) \,\,\,\,s.t. \; \hat{\bm{t}}_i^* = \underset{\bm{t}\in \mathcal{T}}{\arg\max}\; f(\bm{x}_i,\bm{t}).
\end{equation}
%where $\hat{\bm{t}}_i^*$ denotes the predicted optimal treatment of the $i$-th instance.
%
%With a deterministic policy where the treatment with highest $\pi(\bm{t}|\bm{x})$ is always selected, $\hat{\bm{t}}_i^* = \underset{\bm{t}_i'\in \mathcal{T}}{\arg\max}\; \pi(\bm{t}_i'|\bm{x}_i)$ .
%
When we adopt the setting of stochastic preference, it leads to another variant of Eq.~\ref{eq:state} as:
\begin{equation}
\label{eq:obj2sto}
	\underset{f}{\arg\max}\; \frac{1}{N}\sum_{i=1}^N\sum_{\bm{t}\in\mathcal{T}} \pi_i^s(\bm{t};f)y_i(\bm{t}).
\end{equation}
%
%
%With this in mind, existing methods estimate all the potential outcomes $y_i(\bm{t}),\;\forall \bm{t}\in \mathcal{T}$ and recommend treatments based on the those.
%

%To resolve this problem, we propose to reformulate the problem of optimal personalized treatment decision as a learning to rank (LETOR) problem.
%%
%The proposed framework maximizes the posterior probability that we rank $(\bm{x}_i,\bm{t})$ before $(\bm{x}_j,\bm{t}')$ if $y_i(\bm{t}) >y_j(\bm{t}')$.
%%
%To accomplish this, a ranking function $f:(\bm{x},\bm{t})\rightarrow \mathds{R}$ is learned, which can assign ranking score to instance-treatment pairs according to their corresponding potential outcomes.
%\begin{equation}
%		\underset{\pi}{\arg\max}\; \frac{1}{N}\sum_{i=1}^N G(l(\pi_f(r)))D(r),
%\end{equation}
%We propose Learning to Deconfound with BPR loss.
%%
%Existing propensity score based causal inference models adopt the idea of supervised learning.
%%
%In particular, the \textit{propensity score} $Pr(t=1|\bm{x})$ is often predicted by the observed features.
%
%However, the population of each treatment group can be significantly different. A better way to deal with this problem is learning to rank units with their propensity.
%When the treatment variable $t$ is binary, given the confounders $\bm{z}$, the propensity score is defined as $Pr(t=1|\bm{z})$.
%Given a pair of units $(i,j)$ with $t_i=1, t_j=0$, we learn a function to predict the propensity such that $\hat{Pr}(t=1|\bm{z}_i)>\hat{Pr}(t=1|\bm{z}_j)$.
%%
%In this work, we parameterize the propensity score $Pr(t=1|\bm{z})$ with function $f_{PS}(\bm{z};\bm{\theta})$.
%%
%Inspired by the Bayesian Personalized Ranking (BPR)~\cite{rendle2009bpr} model for implicit feedback, we propose the Bayesian Ranking for Potential Outcomes (BRPO) model to solve the problem of personalized optimal treatment assignment.
%
Then we analyze the relationship between optimal solution of the problems in Eq.~\ref{eq:obj2},~\ref{eq:obj2sto}, and a subset of the functional space of ranking functions.
%
We start with the definition of consistency.
\begin{def}\textbf{Consistency. }
	Given the domain of outcomes $\mathcal{Y}$ and a ranking function $f$, if $y_i(\bm{t})>y_j(\bm{t}')$, we say $f$ is consistent with $\mathcal{Y}$ iff $f(\bm{x}_i,\bm{t})> f(\bm{x}_j,\bm{t}'), \forall \bm{x}_i,\bm{x}_j\in \mathcal{X} \;and\; \bm{t},\bm{t}'\in\mathcal{T}$.
\end{def}
\noindent We denote the subset of ranking functions that are consistent with $\mathcal{Y}$ as $\mathcal{F}_\mathcal{Y} = \left\{f|f\text{ is consistent with }\mathcal{Y}\right\}$.
%
Then we show that any $f\in \mathcal{F}_{\mathcal{Y}}$ maximizes the objective functions in Eq.~\ref{eq:obj1} and Eq.~\ref{eq:obj2} with the deterministic preference setting (a receiver always chooses the highest ranked treatment) and the objective function in Eq.~\ref{eq:obj2sto} under the stochastic preference setting (receivers choose each treatment with probability based on their preference) with a mild assumption.
% (2) the objective function of the proposed framework upperbounds the intractable objectives in Eq.~\ref{eq:obj1}-\ref{eq:obj2sto}.

\begin{prop}
	\label{prop:deter}
	Given $f\in \mathcal{F}_{\mathcal{Y}}$, then $y_i(\hat{\bm{t}}_i^*)>y_i(\bm{t}), \; \forall \bm{t}\in \mathcal{T}\setminus \hat{\bm{t}}_i^*$, where $\hat{\bm{t}}_i^* = \underset{\bm{t}}{\arg\max}f(\bm{x}_i,\bm{t})$ denotes the highest ranked treatment by $f$ for instance $i$.
\end{prop}
 This can be proved by reductio-ad-absurdum~\cite{chen2009ranking}. Then, following Proposition~\ref{prop:deter}, the highest ranked treatment by any $f\in \mathcal{F}_{\mathcal{Y}}$ is always the optimal individual treatment, namely $\hat{\bm{t}}_i^* = \bm{t}_i^*$. Under deterministic preference setting, we always have
\begin{equation}
	\pi(\bm{t}|\bm{x}_i) = \begin{cases}
	1, \; \bm{t}=\hat{\bm{t}}_i^*=\bm{t}_i^*\\
	0, \; \bm{t} \in \mathcal{T}\setminus\bm{t}_i^*, \\
	\end{cases}
\end{equation}  %$\underset{\bm{t}_i'}{\arg\max}y_i(\bm{t}_i')$
and thus any $f\in \mathcal{F}_{\mathcal{Y}}$ ensures the maximization of the objective in Eq.~\ref{eq:obj2} in this setting.

When it comes to the setting of stochastic preference, we first make a mild assumption about each receivers' stochastic preference: % 1). each individual's policy assigns constant probability for any treatment ranked at the position $r$ as $\pi_i^s(\bm{t}|\bm{x};f) = l(r)$ is a function of the personalized ranking of each treatment and satisfies:
\begin{equation}
\label{eq:sto_poli}
\pi_i^s(\bm{t};f)\ge\pi_i^s(\bm{t}';f)\; \text{iff} \; f(\bm{x}_i,\bm{t})\ge f(\bm{x}_j,\bm{t}').
\end{equation}
Intuitively, this means the probability that a receiver selects a treatment is monotonic with the corresponding inferred ranking score.
%
Under this assumption, we reveal the connection between the optimization problem in Eq.~\ref{eq:obj2sto} and $\mathcal{F}_\mathcal{Y}$ with Proposition~\ref{prop:sto}.
%
\begin{proposition}
	Given $f\in \mathcal{F}_{\mathcal{Y}}$ and a stochastic policy $\pi_i^s$ satisfies Eq.~\ref{eq:sto_poli}, then $f$ maximizes the objective function in Eq.~\ref{eq:obj2sto}.
		\label{prop:sto}
\end{proposition}

\begin{proof}
	Assuming there exists a ranking function $g\not \in \mathcal{F}_{\mathcal{Y}}$ s.t.
	\begin{equation}
	\label{eq:proof_prop2_1}
		\frac{1}{N}\sum_{i=1}^N\sum_{\bm{t}\in\mathcal{T}} \pi_i^s(\bm{t};g)y_i(\bm{t}) > \frac{1}{N}\sum_{i=1}^N\sum_{\bm{t}\in\mathcal{T}} \pi_i^s(\bm{t};f)y_i(\bm{t}), \forall\; f\in \mathcal{F}_{\mathcal{Y}}.
	\end{equation}
	Then there must exist at least an individual $i$ such that at least a pair of treatments $\bm{t}$ and $\bm{t}'$ satisfies $y_i(\bm{t})>y_i(\bm{t}')$ and $g(\bm{x}_i,\bm{t})\le g(\bm{x}_i,\bm{t}')$. According to Eq.~\ref{eq:sto_poli}, this implies that $\pi_i^s(\bm{t};f') \le \pi_i^s(\bm{t}';f')$.
	%
	Thus we can always create a ranking function $f\in \mathcal{F}_{\mathcal{Y}}$ from $g$ as follows. We swap the ranking score as $f(\bm{x}_i,\bm{t})=g(\bm{x}_i,\bm{t}')\ge f(\bm{x}_i,\bm{t}')=g(\bm{x}_i,\bm{t})$. After each swap, denoting the ranking function before and after the swap as $g''$ and $g'$, then we have
	 \begin{equation}
	 \begin{split}
	 	 	&\pi_i^s(\bm{t};g'')y_i(\bm{t}) + \pi_i^s(\bm{t}';g'')y_i(\bm{t}') \\
			\ge\,\, & \pi_i^s(\bm{t};g')y_i(\bm{t}) + \pi_i^s(\bm{t}';g')y_i(\bm{t}'),
	 \end{split}
	 \end{equation}
	 and for other treatments
	 \begin{equation}
	 \sum_{\bm{t}''\in \mathcal{T}\setminus\left\{\bm{t},\bm{t}'\right\}}\pi_i^s(\bm{t}'';g')y_i(\bm{t}) = 	 \sum_{\bm{t}''\in \mathcal{T}\setminus\left\{\bm{t},\bm{t}'\right\}}\pi_i^s(\bm{t}'';g'')y_i(\bm{t}).
	 \end{equation}
%	 \begin{equation}
%	 \begin{split}
%	 & \sum_{(\bm{t},\bm{t}')}\pi_i^s(\bm{t}|\bm{x}_i;f)y_i(\bm{t}) + \pi_i^s(\bm{t}'|\bm{x}_i;f)y_i(\bm{t}') \ge \\ & \sum_{(\bm{t},\bm{t}')} \pi_i^s(\bm{t}|\bm{x}_i;f')y_i(\bm{t}) + \pi_i^s(\bm{t}'|\bm{x}_i;f')y_i(\bm{t}')\\
%	 \end{split}
%	 \end{equation}
Therefore, each swap keeps the objective function in Eq.~\ref{eq:obj2sto} non-decreasing.
We keep doing this until there does not exist such $\bm{t}$ and $\bm{t}'$ and maintain the ranking scores for the other treatments, and we can repeat this process for other individuals.
At the end, we obtain a ranking function $f\in \mathcal{F}_{\mathcal{Y}}$ s.t.
	 \begin{equation}
	 \begin{split}
	 	\frac{1}{N}\sum_{i=1}^N\sum_{\bm{t}\in\mathcal{T}} \pi_i^s(\bm{t};f)y_i(\bm{t}) &\ge ... \ge \frac{1}{N}\sum_{i=1}^N\sum_{\bm{t}\in\mathcal{T}} \pi_i^s(\bm{t};g'')y_i(\bm{t}) \ge \\ \frac{1}{N}\sum_{i=1}^N\sum_{\bm{t}\in\mathcal{T}} \pi_i^s(\bm{t};g')y_i(\bm{t}) & \ge...\ge \frac{1}{N}\sum_{i=1}^N\sum_{\bm{t}\in\mathcal{T}} \pi_i^s(\bm{t};g)y_i(\bm{t}),
	 \end{split}
	 \end{equation}
	 which conflicts with Eq.~\ref{eq:proof_prop2_1}. Therefore, there does not exist such a function $g$, which completes the proof.
%	\begin{equation}
%		\pi_i^s(\bm{t}_i'|\bm{x}_i;f')y_i(\bm{t}_i') > \pi_i^s(\bm{t}_i'|\bm{x}_i;f)y_i(\bm{t}_i')
%	\end{equation}
%	as $\sum_{\bm{t}_i'\in\mathcal{T}}\pi(\bm{t}_i'|\bm{x}_i;\cdot)=1$, thus, there must also exist $\bm{t}_i''\not = \bm{t}_i'$ such that
%	\begin{equation}
%			\pi_i^s(\bm{t}_i''|\bm{x}_i;f')y_i(\bm{t}_i'') < \pi_i^s(\bm{t}_i''|\bm{x}_i;f)y_i(\bm{t}_i'')
%	\end{equation}
\end{proof}

Until now, we have shown that if a ranking function $f$ is consistent with the potential outcome space $\mathcal{Y}$, then with $f$ we can advocate treatments such that conceptual objectives are maximized under both deterministic and stochastic preference settings.
%
Thus, to achieve good performance for \textit{PLU}, we aim to learn a ranking function which can closely approximate any function $f\in \mathcal{F}_{\mathcal{Y}}$.

However, in observational data, only one of the potential outcomes $y_i$ is available for each instance $i$.
%, where $\bm{t}_i$ may or may not be the predicted optimal treatment.
Hence, it is intractable to evaluate the objective functions in Eq.~\ref{eq:obj2} and \ref{eq:obj2sto}.
%
\vspace{-0.1in}
\subsection{From Consistency to Tractable Objective}
\label{subsec:lossvsloss}
In this subsection, we aim to provide guidance for designing tractable objective functions to tackle the problem of \textit{LSPTD}.
Based on the definition of consistency, we first introduce the essential loss, and its tractable counterpart. Then through theoretical analysis we show the two gaps between them.  %introduce a tractable and differentiable objective function for the proposed framework in the next section. This provides guidance for designing tractable objective functions to tackle the problem of LSPTD.

First, based on the definition of $\mathcal{F}_\mathcal{Y}$ (Definition~\ref{def:problem}), we formally introduce the essential loss $\mathcal{L}(f;\mathcal{Y})$ as:
\begin{equation}
\label{eq:essential_loss}
\mathcal{L}_{es}(f;\mathcal{Y}) = \frac{1}{N|\mathcal{T}|}\sum_i\sum_{\bm{t}\in\mathcal{T}}(1-\prod_{\bm{t}':y_i(\bm{t}')\not=y_i(\bm{t})}\mathds{1}((\bm{x}_i,\bm{t}),(\bm{x}_i,\bm{t}');f)),
\end{equation}
where \begin{equation}
	\mathds{1}((\bm{x}_i,\bm{t}),(\bm{x}_j,\bm{t}');f) = \begin{cases}
	\mathds{1}(f(\bm{x}_i,\bm{t})>f(\bm{x}_j,\bm{t}')) & if y_i(\bm{t})>y_j(\bm{t}')\\
	\mathds{1}(f(\bm{x}_i,\bm{t})<f(\bm{x}_j,\bm{t}')) & if y_i(\bm{t})<y_j(\bm{t}').\\
	\end{cases}
\end{equation}
%It worth noting that, in the essential loss (Eq.~\ref{eq:essential_loss}), pairs $((\bm{x}_i,\bm{t}),(\bm{x}_i,\bm{t}'))$ with $y_i(\bm{t}')>y_i(\bm{t})$ are also involved when we consider individual $i$ and treatment $\bm{t}'$.
%where we evaluate the 1-0 loss
%
Similar to the essential loss of ranking functions for normal learning to rank tasks~\cite{chen2009ranking}, it is easy to verify that
\begin{equation}
\mathcal{L}(f;\mathcal{Y}) = 0 \Leftrightarrow f\in \mathcal{F}_{\mathcal{Y}}.
\end{equation}
Therefore, based on Propositions~\ref{prop:deter} and ~\ref{prop:sto}, we can conclude that the ranking function $f$ achieves minimum of the essential loss, and also reaches the maximum of the conceptual losses for the \textit{LSPTD} problem (Eq.~\ref{eq:obj2} and~\ref{eq:obj2sto}).
%
However, in observational data, only one of the potential outcomes is observed for each individual. Therefore, the essential loss cannot be directly evaluated.
%
But we can compare pairs of observed instances to define the tractable loss as:
\begin{equation}
\label{eq:obs_loss}
\begin{split}
\mathcal{L}_{tra}(f;\mathcal{Y}) = \frac{1}{N}\sum_i (1-\prod_{j:y_j\not=y_i}\mathds{1}((\bm{x}_i,\bm{t}_i),(\bm{x}_j,\bm{t}_j);f)).
\end{split}
\end{equation}\\
%
%It worth mentioning that
%
%We can rewrite the essential loss and the tractable loss as expectations  on different populations of the following 1-0 loss:
%\begin{equation}
%\label{eq:1-0}
%\mathcal{L}_{1-0}((\bm{x},\bm{t}),\left\{(\bm{x}',\bm{t}')\right\};f) = 1-\prod_{(\bm{x}',\bm{t}')}\mathds{1}(f(\bm{x},\bm{t})>f(\bm{x}',\bm{t}'))
%\end{equation}
%For each indivudual $i$, the essential loss can be reformed as:
%\begin{equation}
%	\mathds{E}_{\bm{t}\sim Pr(\bm{t})}[\mathds{E}_{\bm{t}'\sim Pr(\bm{t})}\mathcal{L}_{1-0}((\bm{x}_i,\bm{t}))]
%\end{equation}
%on the pairs $((\bm{x},\bm{t}),(\bm{x}',\bm{t}'))$ of observed and counterfactual instances satisfying $\bm{x}=\bm{x}'=\bm{x}_i$ and $y_i(\bm{t}')<y_i(\bm{t})$ for each individual $i$ and treatment $\bm{t}$.
%Then we analyze the difference between
We can rewrite the essential loss and the tractable loss as expectations on different populations with the following 1-0 loss:
\begin{equation}
\label{eq:1-0}
\mathcal{L}_{1-0}((\bm{x},\bm{t}),\left\{(\bm{x}',\bm{t}')\right\};f) = 1-\prod_{(\bm{x}',\bm{t}')\in \left\{(\bm{x}',\bm{t}')\right\}}\mathds{1}((\bm{x},\bm{t}),(\bm{x}',\bm{t}');f)
\end{equation}
For each individual $i$, the essential loss can be formed as:
\begin{equation}
\label{eq:ess_1-0}
\mathds{E}_{\bm{t}\sim U(\bm{t})}[\mathcal{L}_{1-0}((\bm{x}_i,\bm{t}),\left\{(\bm{x}_i,\bm{t}')\right\}_{\bm{t}'\not =\bm{t}};f)],
\end{equation}
where $U(\bm{t})$ denotes the uniform distribution of treatments,
%
and the tractable loss is:
\begin{equation}
\label{eq:tra_1-0}
\mathcal{L}_{1-0}((\bm{x}_i,\bm{t}_i),\left\{(\bm{x}_j,\bm{t}_j)\right\}_{j\not =i};f).
\end{equation}
%Intuitively, we can see the main difference between the essential loss (Eq.~\ref{eq:essential_loss}) and the tractable loss (Eq.~\ref{eq:obs_loss}) can be summarized as: (1) minimizing the essential loss learns a ranking function that gives correct rankings of the instances with different treatments of the same individual.
%%
%(2) minimizing the tractable loss leads to a ranking function that ranks observed instances in the correct order.
%
%It is not difficult to find the intermediate loss between them which is also intractable. Formally it is can be written as:
%\begin{equation}
%\label{eq:inter_loss}
%\mathcal{L}_{inter}(f;\mathcal{Y}) = \frac{1}{N}\sum_i(1-\prod_{\bm{t}':y_i(\bm{t}')<y_i(\bm{t})}\mathds{1}(f(\bm{x}_i,\bm{t}_i)>f(\bm{x}_i,\bm{t}')))
%\end{equation}
%Then we can analyze the difference between the essential loss (Eq.~\ref{eq:essential_loss}) and the tractable loss (Eq.~\ref{eq:obs_loss}) through comparing them with the intermediate loss (Eq.~\ref{eq:inter_loss}).
%Compared to the essential loss, for each individual $i$, the tractable loss only evaluates the 1-0 loss $1-\prod_{\bm{t}'}\mathds{1}(f(\bm{x},\bm{t})>f(\bm{x}',\bm{t}'))$ on pairs of observed instances $((\bm{x}_i,\bm{t}_i),(\bm{x}_j,\bm{t}_j))$ satisfying $y_j<y_i$ for each individual $i$.
%
%Similarly, the pairs $((\bm{x}_i,\bm{t}_i),(\bm{x}_j,\bm{t}_j))$ where $y_i>y_j$ are also considered in Eq.~\ref{eq:obs_loss} if we swap the value of $i$ and $j$.
%Therefore, we can summarize the differences between them for each individual $i$ as:
%\begin{itemize}
%	\item The tractable loss only considers the observed treatment $\bm{t}_i$ but the essential loss includes all treatments.
%	\item The tractable loss involves all other observed instances $(\bm{x}_j,\bm{t}_j), j\not=i$ while the essential loss considers all counterfactual instances of the $i$-th individual, $(\bm{x}_i,\bm{t}), \bm{t}\not=\bm{t}_i$.
%\end{itemize}
%In Eq.~\ref{eq:essential_loss}, for each individual $i$, we evaluate the 1-0 loss on each treatment $\bm{t}\in\mathcal{T}$ but in Eq.~\ref{eq:obs_loss}, we only consider the observed treatment $\bm{t}_i$. More formally, we know that in Eq.~\ref{eq:inter_loss}, given an individual $i$, we approximate $\mathds{E}_{\bm{t}}[\mathds{E}_{\bm{t}'}[\mathds{1}_i(\bm{t},\bm{t}')]]$ with $\mathds{E}_{\bm{t}'}[\mathds{1}_i(\bm{t},\bm{t}')]$, where $\bm{t}'\in\left\{\bm{t}'|y_i(\bm{t}')<y_i(\bm{t})\right\}$ and $\mathds{1}_i(\bm{t},\bm{t}')$ is short for $\mathds{1}(f(\bm{x}_i,\bm{t}_i)>f(\bm{x}_i,\bm{t}'))$. In short, we dropped the outer expectation over all possible treatments.
%%
%This gap has been well studied in the literature of causal inference and often mitigated by inverse propensity score weighting~\cite{hirano2001estimation,rosenbaum1983central}.%
%	
%Then we analyze the second gap.
%%
%%In Eq.~\ref{eq:obs_loss}, for each instance $i$, we replace the counterfactual counterparts of the same instance $(\bm{x}_i,\bm{t}'),\bm{t}':y_i(\bm{t}')<y_i$ with other observed instances $(\bm{x}_j,\bm{t}_j), y_j<y_i$.
%%
%Formally, in Eq.~\ref{eq:obs_loss}, the expectation $\mathds{E}_{\bm{t}':y_i(\bm{t}')<y_i(\bm{t})}[\mathds{1}_i(\bm{t},\bm{t}')]$ is approximated by $\mathds{E}_{j:y_i<y_i}[\mathds{1}_{ij}]$ where $\mathds{1}_{ij}$ signifies $\mathds{1}(f(\bm{x}_i,\bm{t}_i)>f(\bm{x}_j,\bm{t}_j))$.
%%
%In other words, the expectation over the distribution of counterfactual $Pr(\bm{x}_i,\bm{t}'), \bm{t}'\in\left\{\bm{t}'|y_i(\bm{t}')<y_i\right\}$ is approximated by that on the observed $Pr(\bm{x}_j,\bm{t}_j), j\in\left\{j|y_j<y_i\right\}$.
%Formally, we can write the second gap as the divergence for each instance $i$:
%\begin{equation}
%\label{eq:2nd_gap}
%D(Pr(\bm{z}_j)||Pr(\bm{z}_i(\bm{t}))), j\in\left\{j|y_j<y_i\right\}, \bm{t}\in\left\{\bm{t}|y_i(\bm{t})<y_i\right\}
%\end{equation}
%
%The first difference can be approximately reduced by the technique of inverse propensity score weighting~\cite{hirano2001estimation,rosenbaum1983central} where we weight the loss corresponding to each individual with $\frac{1}{Pr(\bm{t}_i|\bm{x}_i)}$.
%
We can find two differences between the essential loss and the tractable loss by comparing Eq.~\ref{eq:ess_1-0} and Eq.~\ref{eq:tra_1-0}: (1) The tractable loss replaces the expectation over all treatments with the observed treatment. (2) The tractable loss replaces counterfactual instances with other observed instances.
%(1)  (2)
The first difference is known as the treatment selection bias and has been well studied in the literature of causal inference and is often mitigated by inverse propensity score weighting~\cite{hirano2001estimation,rosenbaum1983central}.
%
The second difference would be smaller if the difference between the distribution of the observed instances and that of the counterfactual instances, i.e., $D(Pr((\bm{x}_i,\bm{t}_i))||Pr((\bm{x}_i,\bm{t}))), \bm{t}\not=\bm{t}_i, i=1,...,N$ is smaller.
%
However, we cannot directly do this in the original feature and treatment space.
%Intuitively, the second difference means that: (1) We are training ranking functions by comparing pairs as $(\bm{x}_i,\bm{t}_i),(\bm{x}_j,\bm{t}_j),i\not=j$, i.e. observed instances from different individuals. In this case, the difference between the outcomes of instances can be caused by both features and treatments.
%%%
%(2) But the task of LSPTD requires us to rank the pairs $((\bm{x},\bm{t}),(\bm{x},\bm{t}'),\bm{t}\not=\bm{t}')$, namely of observed and counterfactual instances of the same individual. Here, only the treatments make a difference on the outcome.
%%
%Therefore, we need to translate the influence of features on the outcomes to that of treatments.
%Intuitively, the differences mean we are training ranking functions by comparing pairs as $(\bm{x}_i,\bm{t}_i),(\bm{x}_j,\bm{t}_j),i\not=j$, i.e. observed instances from different individuals. In this case, the difference between the outcomes of instances can be caused by both features and treatments.
%%
%But the task of LSPTD requires us to rank the pairs $((\bm{x},\bm{t}),(\bm{x},\bm{t}'),\bm{t}\not=\bm{t}')$, namely of observed and counterfactual instances of the same individual. Here, only the treatments make a difference on the outcome.
%
%This observation motivates us to design a framework where we can translate the influence of features on the outcomes to that of treatments.
%
%Traditionally, as the features and the treatments from different spaces, methods are proposed to reweight observed instances
%%
%However, it is challenging to narrow the second aforementioned difference because the counterfactual outcomes cannot be obtained from observational data.
%
In the next section, we will introduce the proposed \textit{LETORPO} framework that allows us to minimize the aforementioned divergence in the representation space.

